You have been warned: Abusing 5G's Warning and Emergency Systems

The Public Warning System (PWS) is an essential part of cellular networks and a country's civil protection. Warnings can notify users of hazardous events (e.g., floods, earthquakes) and crucial national matters that require immediate attention. PWS attacks disseminating fake warnings or concealing precarious events can have a serious impact, causing fraud, panic, physical harm, or unrest to users within an affected area. In this work, we conduct the first comprehensive investigation of PWS security in 5G networks. We demonstrate five practical attacks that may impact the security of 5G-based Commercial Mobile Alert System (CMAS) as well as Earthquake and Tsunami Warning System (ETWS) alerts. Additional to identifying the vulnerabilities, we investigate two PWS spoofing and three PWS suppression attacks, with or without a man-in-the-middle (MitM) attacker. We discover that MitM-based attacks have more severe impact than their non-MitM counterparts. Our PWS barring attack is an effective technique to eliminate legitimate warning messages. We perform a rigorous analysis of the roaming aspect of the PWS, incl. its potentially secure version, and report the implications of our attacks on other emergency features (e.g., 911 SIP calls). We discuss possible countermeasures and note that eradicating the attacks necessitates a scrupulous reevaluation of the PWS design and a secure implementation.

==> sections/7.further-discussion.tex <==
\section{Further Discussion}

\textit{Is it a relevant threat if an attacker sends forged warning messages to an individual user or a small group of users, or only to a large crowd?} We believe that the more users receive fake messages the merrier the impact becomes as mass panic may lead to hazardous incidents such as physical harm. In fact, the attacker's objective is to affect as many people as possible within a dense, limited or overcrowded space for a specific time window. Geographically speaking,~\cite{Lee19:spoofing-alerts-lte} has shown that four LTE base stations can easily impact a stadium with an approximate capacity of $50,000$ seats. On such a level, we believe that the attacks can turn into an alarming risk.

\textit{Is it a relevant threat if an attacker can suppress warning messages to an individual user or a small group of users, or only to a large crowd?} Similar to spoofing bogus messages, message suppression aims to influence as many network subscribers as possible. Not allowing many users to get notifications about an emergency could also lead to life threatening scenarios. In addition, based on Section~\ref{exploitation}, we consider suppression more trivial than any spoofing approaches, hence increasing the threat level. 

\textit{Could PWS Security be a mandatory requirement?} Protection of warning notifications and users against attackers are subject to regulatory policies. According to 3GPP~\cite{3gpp.133.969}, the requirements for PWS security are optional since there are regions and countries that do not require or aim to deploy this feature any time soon (such as US and Japan). Therefore, without outright and compulsory security, networks will remain exposed to warning spoofing and suppression.

\textit{Are SMS-based warnings affected?} On 5G, the SMS~\cite{3gpp.123.040} deliveries are either over IMS (SIP-based) or over NAS. The UE receives a specific paging message for an SMS service and then the UE enters the RRC-Connected state while sending a Service Request. Then, the network delivers the SMS notifications using the downlink transmission. We ran dedicated experiments for the SMS-based warnings. Since our suppression attacks disallow connection to the legitimate network, the victim-UE will not be able to receive paging messages and consequently the SMS-based warning. Regarding spoofing SMS warnings and DoS, past works~\cite{Hua16:IMS-threats, Hongil15:Breaking-voLTE, Hua16:IMS-SMS, Traynor12} have demonstrated the weakness of SMS over IMS on LTE which may also affect 5G in certain cases. On the other hand, according to 3GPP~\cite{3gpp.33.501}, SMS over NAS implements encryption and integrity-protection when the UE has already activated NAS security with the AMF. However, more testing is required to verify its robustness on 5G against spoofing as~\cite{Kim19:touching-untouchables, Park22:Negative-test} have confirmed SMS over NAS weaknesses on LTE.
